LERC: Coordinated Cache Management for Data-Parallel Systems

Memory caches are being aggressively used in today's data-parallel frameworks such as Spark, Tez and Storm. By caching input and intermediate data in memory, compute tasks can witness speedup by orders of magnitude. To maximize the chance of in-memory data access, existing cache algorithms, be it recency- or frequency-based, settle on cache hit ratio as the optimization objective. However, unlike the conventional belief, we show in this paper that simply pursuing a higher cache hit ratio of individual data blocks does not necessarily translate into faster task completion in data-parallel environments. A data-parallel task typically depends on multiple input data blocks. Unless all of these blocks are cached in memory, no speedup will result. To capture this all-or-nothing property, we propose a more relevant metric, called effective cache hit ratio. Specifically, a cache hit of a data block is said to be effective if it can speed up a compute task. In order to optimize the effective cache hit ratio, we propose the Least Effective Reference Count (LERC) policy that persists the dependent blocks of a compute task as a whole in memory. We have implemented the LERC policy as a memory manager in Spark and evaluated its performance through Amazon EC2 deployment. Evaluation results demonstrate that LERC helps speed up data-parallel jobs by up to 37% compared with the widely employed least-recently-used (LRU) policy.

==> relatedwork.tex <==
%!TEX root = main.tex
\section{Related Work}
\label{sec:related}

\noindent \textbf{Traditional Caching on a Single Machine.}
Memory caching has a long history and has been widely employed in storage systems \cite{chen1994raid}, databases \cite{stonebraker1981operating}, file systems \cite{nelson1988caching}, web servers \cite{cao1997cost}, operating systems \cite{baker2011megastore}, and processors \cite{henning2000spec}. Over the years, a vast amount of caching algorithms have been proposed. These algorithms run on a single machine and can be broadly divided into two categories:

\emph{Recency/frequency-based policies:} LRU \cite{mattson1970evaluation} and LFU \cite{aho1971principles} are the two widely used caching algorithms. As shown in Section \ref{sec:background}, neither algorithm adapts well to the data access pattern in data analytic clusters even though they are simple to implement. %Recency and frequency have also been combined in many caching policies. For example, Least Recently/Frequently Used (LRFU) \cite{lee2001lrfu} and its adaptive version \cite{lee1999existence} dynamically adjust between LRU and LFU. 

\emph{Hint-based policies:} Many cache policies evict/prefetch data blocks through hints from applications \cite{cao1996implementation,patterson1995informed}, which are provided by the programmers to indicate what data will be referenced again and when. Nevertheless, inserting such hints can be difficult to the programmer, who has to carefully examine the underlying data access pattern. %As an alternative approach, hints can also be inserted by compliers [15] or through predictions [20]. Yet, these techniques cannot handle complex, input-dependent access patterns.

% To summarize, traditional caching policies do not assume application semantics, nor do they factor in the data parallel nature of cluster applications.

%\subsection{In-memory caches at scale}

%Thanks to the recent technology advancements, in-memory storage and cache systems have scaled out to large clusters, ranging from specialized applications to general purpose data processing. Example systems for the specialized applications include Memcached \cite{memcached} and Redis \cite{redis}, which provide in-memory key-value stores with high availability for large scale web applications. RAMCloud [36] proposes to persist all data in cluster RAM and is particularly suitable for web servers. Megastore \cite{baker2011megastore} offers a distributed in-memory storage with strong consistency for interactive online services. MemSQL \cite{memsql} comes as a real-time, in-memory database for SQL analytics.

%In-memory caches also serve as a critical component of general purpose data parallel systems. Frameworks like Spark \cite{zaharia2012resilient}, Piccolo \cite{power2010piccolo}, Tez \cite{saha2015apache}, M3R \cite{shinnar2012m3r:}, and Grappa \cite{nelson2015latency} all support caching intermediate data in memory. The recently proposed Alluxio \cite{li2014tachyon} pushes the boundary further by enabling in-memory data sharing across multiple frameworks. %Similar features have also been projected in HDFS Caching.

\vspace{.4em}
\noindent \textbf{Cache Management in Parallel Processing Systems.}
Despite the significant performance impact of memory caches, cache management remains a relatively unchartered territory in data parallel systems. Prevalent parallel frameworks (e.g., Spark \cite{zaharia2012resilient}, Tez \cite{saha2015apache}, and Tachyon \cite{li2014tachyon}) simply employ LRU to manage cached data on cluster machines, which results in a significant performance loss \cite{ananthanarayanan2012pacman:,xu2016memtune:}.

To our knowledge, the recently proposed MemTune \cite{xu2016memtune:} is the only caching system that leverages the application semantics. MemTune dynamically adjusts the memory share for task computation and data caching in Spark and evicts/prefetches data as needed. As opposed to our proposal that accounts for the entire DAG and its dependencies, MemTune only considers locally dependent blocks of currently runnable tasks. Moreover, when it comes to a multi-tenant environment, the complexity of MemTune is also multiplied, as MemTune keeps track of all the submitted DAGs and traverses them at runtime to search for the downstream tasks whenever a task completes. In comparison, LRC parses the job DAG upon job submission and only sends the reference count profile to the corresponding worker node. The reference count updating message is light and simple compared to the DAG structure itself, and can be easily applied to any DAG-based system and even heterogeneous environments running different systems, like Tachyon \cite{li2014tachyon}. 

Recent works \cite{pu2016fairride:,kunjir2015robus} have also studied the problem of cache allocation for multiple users with shared files in clusters, where fairness is the main objective to achieve. We view these works orthogonal to our proposed research. Once the cache space of each application has been allocated by some fair sharing policies, we can leverage the application-specific semantics for efficient cache management.

\begin{comment}
Cache management is a well studied topic. There have been many studies on classical cache replacement policies, such as LRU and LFU, which have been widely adopted in conventional caches \cite{o1993lru}, \cite{breslau1999web}. The expected performance of LRU is analyzed in \cite{che2002hierarchical} by approximating the cache eviction time -- the time since the last request after which an item will be evicted from the cache. There are also works \cite{lee2001lrfu}\cite{karedla1994caching} that combine LRU and LFU to adapt to the variant data access pattern. 

Recently, a number of cache management mechanisms specially tailored for the distributed in-memory processing systems have also been designed. Tachyon \cite{li2014tachyon} provides a distributed memory layer to share data across multiple frameworks. CRAMM \cite{yang2006cramm} offers dynamic JVM heap management to accommodate variant compute demands. MegaStore \cite{baker2011megastore} specially tunes the cache management to provide consistent storage guarantees for interactive online applications. The LRC policy proposed in this paper differentiates from them in that LRC factors in the scheduling information and relies on data dependency to improve the cache management.

FairRide \cite{pu2016fairride:} offers a solution to guarantee the fairness of cache sharing in multi-tenant in-memory processing systems: probabilistically block requests to the data cached by other users. LRC strives to make the best use of the available cache space of each user, thus it is orthogonal and can be applied atop FairRide.

MEMTUNE \cite{xu2016memtune:} is the work most related to our study as it also leverages the DAG information to guide the cache management. Specifically, it focuses on dynamically adjusting the memory fraction for computation and caching, as well as prefetching the data of the next compute stage in the DAG. Compared to MemTune, LRC keeps a broader horizon of the future data dependency by aggregating the reference count in the entire job, rather than only one stage afterwards. Besides, the practicality of MemTune is hindered in a multi-tenant environment, as for a shared memory pool, individual adjustment to the memory fraction of computation/cache is inapplicable. LRC can be naturally extended to the multi-tenant systems, and can also easily assign priority to different users by normalizing the reference count.
\end{comment}

